The inner structure of boundary quotients of right LCM semigroups

We study distinguished subalgebras and automorphisms of boundary quotients arising from algebraic dynamical systems $(G,P,\theta)$. Our work includes a complete solution to the problem of extending Bogolubov automorphisms from the Cuntz algebra in $2 \leq p<\infty$ generators to the $p$-adic ring $C^*$-algebra. For the case where $P$ is abelian and $C^*(G)$ is a maximal abelian subalgebra, we establish a picture for the automorphisms of the boundary quotient that fix $C^*(G)$ pointwise. This allows us to show that they form a maximal abelian subgroup of the entire automorphism group. The picture also leads to the surprising outcome that, for integral dynamics, every automorphism that fixes one of the natural Cuntz subalgebras pointwise is necessarily a gauge automorphism. Many of the automorphisms we consider are shown to be outer.

==> bib.tex <==

%\begin{bibdiv}
\begin{biblist}

\bib{ABLS}{article}{
author={Afsar, Zahra},
author={Brownlowe, Nathan},
author={Larsen, Nadia S.},
author={Stammeier, Nicolai},
title={Equilibrium states on right LCM semigroup $C^*$-algebras},
journal={Int. Math. Res. Not.},
year={2017 (advance article)},
doi={\href{https://doi.org/10.1093/imrn/rnx162}{10.1093/imrn/rnx162}},
%note={preprint, \href{https://arxiv.org/abs/1611.01052}{arxiv:1611.01052}},
}


\bib{ACR}{article}{%MR3749344,
author={Aiello, Valeriano},
author={Conti, Roberto},
author={Rossi, Stefano},
title={A look at the inner structure of the $2$-adic ring $C^*$-algebra and its automorphism groups},
   JOURNAL = { Publ. Res. Inst. Math. Sci.},
    VOLUME = {54},
      YEAR = {2018},
    NUMBER = {1},
     PAGES = {45--87},
     ISSN = {0034-5318},
  % MRCLASS = {46L40 (46L05)},
 % MRNUMBER = {3749344},
%MRREVIEWER = {Daniele Puglisi},       
   DOI = {\href{https://doi.org/10.4171/PRIMS/54-1-2 }{10.4171/PRIMS/54-1-2 }},
}

\bib{ACR2}{article}{
author={Aiello, Valeriano},
author={Conti, Roberto},
author={Rossi, Stefano},
title={Diagonal automorphisms of the $2$-adic ring $C^*$-algebra},
journal={Q. J. Math.},
    VOLUME = {69},
    issue={3},
      YEAR = {2018},
%    NUMBER = {2},
     PAGES = {815--833},
       DOI = {\href{https://doi.org/10.1093/qmath/hax064}{10.1093/qmath/hax064}},
}

\bib{AD}{article}{%MR919508,
    AUTHOR = {Anantharaman-Delaroche, Claire},
     TITLE = {Syst\`{e}mes dynamiques non commutatifs et moyennabilit\'{e}},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {279},
      YEAR = {1987},
    NUMBER = {2},
     PAGES = {297--315},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L55 (22D25 22D40 43A07 43A35)},
 % MRNUMBER = {919508 (89f:46127)},
%MRREVIEWER = {Elliot C. Gootman},
       DOI = {\href{http://dx.doi.org/10.1007/BF01461725}{10.1007/BF01461725}},
}

\bib{ADR}{book}{%MR1799683,
    AUTHOR = {Anantharaman-Delaroche, Claire},
    AUTHOR = {Renault, Jean},
     TITLE = {Amenable groupoids},
    SERIES = {Monographies de L'Enseignement Math\'{e}matique},% [Monographs of L'Enseignement Math\'ematique]
    VOLUME = {36},
      NOTE = {With a foreword by Georges Skandalis and Appendix B by E. Germain},
 PUBLISHER = {L'Enseignement Math\'{e}matique, Geneva},
      YEAR = {2000},
     PAGES = {196},
      ISBN = {2-940264-01-5},
   %MRCLASS = {22A22 (22D25 43A07 46L05 46L10 46L80)},
  %MRNUMBER = {1799683 (2001m:22005)},
%MRREVIEWER = {Robert S. Doran},
}

\bib{AM}{article}{
author={Albandik, Suliman},
author={Meyer, Ralf},
title={Product systems over Ore monoids},
note={preprint \href{http://arxiv.org/abs/1502.07768}{arxiv:1502.07768}},
}

\bib{AR}{incollection} {%MR1491110,
    AUTHOR = {Arzumanian, Victor},
    AUTHOR = {Renault, Jean},
     TITLE = {Examples of pseudogroups and their C*-algebras},
 BOOKTITLE = {Operator algebras and quantum field theory ({R}ome, 1996)},
     PAGES = {93--104},
 PUBLISHER = {Int. Press, Cambridge, MA},
      YEAR = {1997},
  % MRCLASS = {46L05},
 % MRNUMBER = {1491110 (99a:46101)},
%MRREVIEWER = {Siegfried Echterhoff},
}

\bib{AS}{article}{%MR1258035,
    AUTHOR = {Archbold, Robert J.},
    AUTHOR = {Spielberg, Jack S.},
     TITLE = {Topologically free actions and ideals in discrete C*-dynamical systems},
   JOURNAL = {Proc. Edinburgh Math. Soc. (2)},
 % FJOURNAL = {Proceedings of the Edinburgh Mathematical Society. Series II},
    VOLUME = {37},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {119--124},
      ISSN = {0013-0915},
%     CODEN = {PRMSA3},
 %  MRCLASS = {46L55},
  %MRNUMBER = {1258035 (94m:46101)},
%MRREVIEWER = {Yasuyuki Kawahigashi},
       DOI = {\href{http://dx.doi.org/10.1017/S0013091500018733}{10.1017/S0013091500018733}},
}

\bib{Arveson}{book}{%arveson2006short,
  title={A short course on spectral theory},
  author={Arveson, William},
  volume={209},
  year={2006},
  publisher={Springer Science \& Business Media}
}


\bib{Bae}{article}{%MR0009955,
    AUTHOR = {Baer, Reinhold},
     TITLE = {Groups without proper isomorphic quotient groups},
   JOURNAL = {Bull. Amer. Math. Soc.},
  %FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {50},
      YEAR = {1944},
     PAGES = {267--278},
      ISSN = {0002-9904},
  % MRCLASS = {20.0X},
 % MRNUMBER = {0009955 (5,228a)},
%MRREVIEWER = {I. Kaplansky},
}

\bib{barlak}{thesis}{
    AUTHOR = {Barlak, Sel\c{c}uk},
     TITLE = {On the $K$-theory of Crossed Product {$C^*$}-algebras by Actions of $\mathbb Z^n$},
    SCHOOL = {Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster},
      YEAR = {2014},
}

\bib{barlak15}{article}{
	AUTHOR={Barlak, Sel\c{c}uk},
	TITLE={On the spectral sequence associated with the Baum-Connes Conjecture for $\mathbb Z^n$},
	NOTE={preprint, \href{http://arxiv.org/abs/1504.03298}{arxiv.org:1504.03298}},
	YEAR={2015},
}

\bib{BL1}{article} {%MR3672919,
    AUTHOR = {Barlak, Sel\c{c}uk},
    author={Li, Xin},
     TITLE = {Cartan subalgebras and the {UCT} problem},
   JOURNAL = {Adv. Math.},
%  FJOURNAL = {Advances in Mathematics},
    VOLUME = {316},
      YEAR = {2017},
     PAGES = {748--769},
      ISSN = {0001-8708},
%   MRCLASS = {46L10},
 % MRNUMBER = {3672919},
       DOI = {\href{http://dx.doi.org/10.1016/j.aim.2017.06.024}{10.1016/j.aim.2017.06.024}},
    %   URL = {http://dx.doi.org/10.1016/j.aim.2017.06.024},
}


\bib{BL2}{article}{
AUTHOR = {Barlak, Sel\c{c}uk},
    author={Li, Xin},
     TITLE = {Cartan subalgebras and the {UCT} problem, II},
  note={preprint, \href{https://arxiv.org/abs/1704.04939}{arxiv:1704.04939}},   
}


\bib{BOS1}{article}{
	AUTHOR={Barlak, Sel\c{c}uk},
	author={Omland, Tron},
	author={Stammeier, Nicolai},
	TITLE={On the K-theory of $C^*$-algebras arising from integral dynamics},
	JOURNAL = {Ergodic Theory Dynam. Systems},
  %FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {38},
      YEAR = {2018},
    NUMBER = {3},
     PAGES = {832--862},
      ISSN = {0143-3857},
  % MRCLASS = {37A55 (46L35)},
%  MRNUMBER = {3784245},
       DOI = {\href{https://doi.org/10.1017/etds.2016.63}{10.1017/etds.2016.63}},
%       URL = {https://doi.org/10.1017/etds.2016.63},
}


\bib{BarSza1}{article}{
author={Barlak, Sel\c{c}uk},
author={Szab\'{o}, G\'{a}bor},
title={Sequentially split $*$-homomorphisms between $C^*$-algebras},
note={preprint, \href{http://arxiv.org/abs/1510.04555}{arxiv:1510.04555}},
%year={2015},
}


\bib{Ber1}{article}{%MR716835,
    AUTHOR = {Berend, Daniel},
     TITLE = {Multi-invariant sets on tori},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {280},
      YEAR = {1983},
    NUMBER = {2},
     PAGES = {509--532},
      ISSN = {0002-9947},
   %  CODEN = {TAMTAM},
   %MRCLASS = {11K06 (11K55 28D10 54A15)},
  %MRNUMBER = {716835 (85b:11064)},
%MRREVIEWER = {G{\'e}rard Rauzy},
       DOI = {\href{http://dx.doi.org/10.2307/1999631}{10.2307/1999631}},
  %     URL = ,
}

\bib{Ber2}{article}{%MR760973,
    AUTHOR = {Berend, Daniel},
     TITLE = {Multi-invariant sets on compact abelian groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {286},
      YEAR = {1984},
    NUMBER = {2},
     PAGES = {505--535},
      ISSN = {0002-9947},
   %  CODEN = {TAMTAM},
   %MRCLASS = {22D40 (11J61 11J69)},
  %MRNUMBER = {760973 (86e:22009)},
%MRREVIEWER = {Justin Peters},
       DOI = {\href{http://dx.doi.org/10.2307/1999808}{10.2307/1999808}},
 %      URL = ,
}

\bib{BD}{article}{%MR0365157,
    AUTHOR = {Bunce, John W.},
    AUTHOR = {Deddens, James A.},
     TITLE = {A family of simple C*-algebras related to weighted shift operators},
   JOURNAL = {J. Funct. Anal.},
    VOLUME = {19},
      YEAR = {1975},
     PAGES = {13--24},
  % MRCLASS = {46LXX (47C10)},
 % MRNUMBER = {0365157 (51 \#1410)},
%MRREVIEWER = {R. G. Douglas},
}

\bib{Bla}{book} {%MR2188261,
    AUTHOR = {Blackadar, Bruce},
     TITLE = {Operator Algebras},
    SERIES = {Encyclopaedia of Mathematical Sciences},
    VOLUME = {122},
     % NOTE = {Theory of C*-Algebras and von Neumann Algebras, Operator Algebras and Non-commutative Geometry, III},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2006},
     PAGES = {xx+517},
      ISBN = {978-3-540-28486-4; 3-540-28486-9},
  % MRCLASS = {46L05 (46L10 46L80)},
 % MRNUMBER = {2188261 (2006k:46082)},
%MRREVIEWER = {Paul Jolissaint},
}

\bib{Bri1}{article} {%MR2124335,
    AUTHOR = {Brin, Matthew G.},
     TITLE = {On the {Z}appa-{S}z\'ep product},
   JOURNAL = {Comm. Algebra},
  %FJOURNAL = {Communications in Algebra},
    VOLUME = {33},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {393--424},
      ISSN = {0092-7872},
    % CODEN = {COALDM},
  % MRCLASS = {20N02 (20M99)},
 % MRNUMBER = {2124335},
%MRREVIEWER = {V{\={\i}}tal{\={\i}}{\u\i} M. Usenko},
       DOI = {\href{http://dx.doi.org/10.1081/AGB-200047404}{10.1081/AGB-200047404}},
  %     URL = {http://dx.doi.org/10.1081/AGB-200047404},
}

\bib{BOFS}{article}{
	AUTHOR = {Brown, Jonathan H.},
  AUTHOR = {Orloff Clark, Lisa},
	AUTHOR = {Farthing, Cynthia},
  AUTHOR = {Sims, Aidan},
  TITLE = {Simplicity of algebras associated to \'{e}tale groupoids},
  JOURNAL = {Semigroup Forum},
%  FJOURNAL = {Semigroup Forum},
    VOLUME = {88},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {433--452},
      ISSN = {0037-1912},
 %  MRCLASS = {Preliminary Data},
%  MRNUMBER = {3189105},
       DOI = {\href{http://dx.doi.org/10.1007/s00233-013-9546-z}{10.1007/s00233-013-9546-z}},
}

\bib{BO}{book} {%MR2391387,
    AUTHOR = {Brown, Nathanial P.},
    AUTHOR = {Ozawa, Narutaka},
     TITLE = {C*-Algebras and Finite-Dimensional Approximations},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {88},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, RI},
      YEAR = {2008},
     PAGES = {xvi+509},
      ISBN = {978-0-8218-4381-9; 0-8218-4381-8}
  % MRCLASS = {46L05 (43A07 46-02 46L10)},
 % MRNUMBER = {2391387 (2009h:46101)},
%MRREVIEWER = {Mikael R{\o}rdam},
}

\bib{BaHLR}{article}{
AUTHOR = {Brownlowe, Nathan},
author={an Huef, Astrid},
author={Laca, Marcelo},
author={Raeburn, Iain},
     TITLE = {Boundary quotients of the {T}oeplitz algebra of the affine semigroup over the natural numbers},
   JOURNAL = {Ergodic Th. Dynam. Sys.},
%  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {32},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {35--62},
      ISSN = {0143-3857},
   %MRCLASS = {46L55},
  %MRNUMBER = {2873157 (2012j:46101)},
%MRREVIEWER = {Valentin Deaconu},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385710000830}{10.1017/S0143385710000830}},
%       URL = ,
}

\bib{BLS1}{article}{
	AUTHOR={Brownlowe, Nathan},
	AUTHOR={Larsen, Nadia S.},	
	AUTHOR={Stammeier, Nicolai},
	TITLE={On $C^*$-algebras associated to right LCM semigroups},
	JOURNAL = {Trans. Amer. Math. Soc.},
    VOLUME = {369},
    NUMBER = {1},
    PAGES = {31--68},
	YEAR={2017},
	DOI={\href{http://dx.doi.org/10.1090/tran/6638}{10.1090/tran/6638}},
}

\bib{BLS2}{article}{
	AUTHOR={Brownlowe, Nathan},
	AUTHOR={Larsen, Nadia S.},	
	AUTHOR={Stammeier, Nicolai},
	TITLE={$C^*$-algebras of algebraic dynamical systems and right LCM semigroups},
	JOURNAL={to appear in Indiana Univ. Math. J. },
	NOTE={preprint available under \href{http://www.iumj.indiana.edu/IUMJ/Preprints/7527.pdf}{IUMJ/Preprints/7527}},
}

\bib{BRRW}{article}{%MR3165249,
    AUTHOR = {Brownlowe, Nathan},
    AUTHOR = {Ramagge, Jacqui}, 
    AUTHOR = {Robertson, David},
    AUTHOR = {Whittaker, Michael F.},
     TITLE = {Zappa-{S}z\'{e}p products of semigroups and their $C^*$-algebras},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {266},
      YEAR = {2014},
    NUMBER = {6},
     PAGES = {3937--3967},
      ISSN = {0022-1236},
  % MRCLASS = {46L05 (20E08)},
 % MRNUMBER = {3165249},
%MRREVIEWER = {C. J. K. Batty},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2013.12.025}{10.1016/j.jfa.2013.12.025}},
 %      URL = {http://dx.doi.org/10.1016/j.jfa.2013.12.025},
}

\bib{BS1}{article}{
author={Brownlowe, Nathan},
author={Stammeier, Nicolai},
 TITLE = {The boundary quotient for algebraic dynamical systems},
   JOURNAL = {J. Math. Anal. Appl.},
 % FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {438},
      YEAR = {2016},
    NUMBER = {2},
     PAGES = {772--789},
  %    ISSN = {0022-247X},
%   MRCLASS = {Preliminary Data},
%  MRNUMBER = {3466063},
       DOI = {\href{http://dx.doi.org/10.1016/j.jmaa.2016.02.015}{10.1016/j.jmaa.2016.02.015}},
   %    URL = {http://dx.doi.org/10.1016/j.jmaa.2016.02.015},
}
}

\bib{CLSV}{article} {%MR2837016,
    AUTHOR = {Carlsen, Toke Meier},
    AUTHOR = {Larsen, Nadia S.},
    AUTHOR = {Sims, Aidan},
    AUTHOR = {Vittadello, Sean T.},
     TITLE = {Co-universal algebras associated to product systems, and gauge-invariant uniqueness theorems},
   JOURNAL = {Proc. Lond. Math. Soc. (3)},
%  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {103},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {563--600},
      ISSN = {0024-6115},
%   MRCLASS = {46L05},
%  MRNUMBER = {2837016 (2012h:46085)},
%MRREVIEWER = {Yangping Jing},
       DOI = {\href{http://dx.doi.org/10.1112/plms/pdq028}{10.1112/plms/pdq028}},
}

\bib{CS}{article} {%MR2563500,
    AUTHOR = {Carlsen, Toke Meier},
    AUTHOR = {Silvestrov, Sergei},
     TITLE = {On the {E}xel crossed product of topological covering maps},
   JOURNAL = {Acta Appl. Math.},
%  FJOURNAL = {Acta Applicandae Mathematicae. An International Survey Journal
%              on Applying Mathematics and Mathematical Applications},
    VOLUME = {108},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {573--583},
      ISSN = {0167-8019},
%     CODEN = {AAMADV},
%   MRCLASS = {46L55 (37B05)},
%  MRNUMBER = {2563500 (2010k:46071)},
%MRREVIEWER = {Masaharu Kusuda},
       DOI = {\href{http://dx.doi.org/10.1007/s10440-008-9372-6}{10.1007/s10440-008-9372-6}},
}

\bib{Car}{article} {%MR2772352,
    AUTHOR = {Carri{\'o}n, Jos{\'e} R.},
     TITLE = {Classification of a class of crossed product C*-algebras associated with residually finite groups},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {260},
      YEAR = {2011},
    NUMBER = {9},
     PAGES = {2815--2825},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L55 (20E26 46L80)},
%  MRNUMBER = {2772352 (2012e:46146)},
%MRREVIEWER = {Nadia S. Larsen},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2011.02.002}{10.1016/j.jfa.2011.02.002}},
}

\bib{CaHR}{article}{
 AUTHOR = {Clark, Lisa Orloff},
  AUTHOR = {an Huef, Astrid},
   AUTHOR = {Raeburn, Iain},
   TITLE = {Phase transition on the Toeplitz algebra of Baumslag-Solitar semigroups},
   journal={to appear in Indiana Univ. Math. J.},
   NOTE = {preprint \href{http://arxiv.org/abs/1503.04873}{arxiv:1503.04873}},
}

\bib{Com}{article} {%MR748991,
    AUTHOR = {Combes, F.},
     TITLE = {Crossed products and {M}orita equivalence},
   JOURNAL = {Proc. London Math. Soc. (3)},
%  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {49},
      YEAR = {1984},
    NUMBER = {2},
     PAGES = {289--306},
      ISSN = {0024-6115},
%     CODEN = {PLMTAL},
%   MRCLASS = {46L55 (46L05)},
%  MRNUMBER = {748991 (86c:46081)},
       DOI = {\href{http://dx.doi.org/10.1112/plms/s3-49.2.289}{10.1112/plms/s3-49.2.289}},
%       URL = ,
}

\bib{connes}{article}{
title={{An analogue of the Thom isomorphism for crossed products by an action of {$\R$}}},
author={Connes, Alain},
year={1981},
journal={Adv. in Math.},
volume={39},
pages={31--55},
}


\bib{Conti}{article}{
AUTHOR={Conti, Roberto},
TITLE={Automorphisms of the UHF algebra that do not extend to the Cuntz algebra},
JOURNAL={ J. Aust. Math. Soc.},
VOLUME={89},
YEAR={2010},
PAGES={309--315},
}

\bib{CHS1}{article}{
AUTHOR={Conti, Roberto},
author={Hong, Jeong Hee},
author={Szyma\'nski, Wojciech},
TITLE={The restricted Weyl group of the Cuntz algebra and shift endomorphisms},
JOURNAL={J. Reine Angew. Math.},
VOLUME={667},
YEAR={2012},
PAGES={177--191},
}

\bib{CHS2}{article}{
AUTHOR={Conti, Roberto},
author={Hong, J. H. },
author={Szyma\'nski, Wojciech},
TITLE={Endomorphisms of graph algebras},
JOURNAL={J. Funct. Anal.},
VOLUME={263},
YEAR={2012},
PAGES={2529--2554},
}

\bib{CHS3}{article}{
AUTHOR={Conti, Roberto},
author={Hong, J. H. },
author={Szyma\'nski, Wojciech},
TITLE={The Weyl group of the Cuntz algebra},
JOURNAL={Adv. Math.},
VOLUME={231},
YEAR={2012},
NUMBER={6},
PAGES={3147--3161},
}

\bib{CHS4}{article}{
AUTHOR={Conti, Roberto},
author={Hong, J. H. },
author={Szyma\'nski, Wojciech},
TITLE={Endomorphisms of the Cuntz Algebras},
JOURNAL={ Banach Center Publ.},
VOLUME={96},
YEAR={2012},
PAGES={81--97},
}


\bib{CHS5}{article}{
AUTHOR={Conti, Roberto},
author={Hong, Jeong Hee},
author={Szyma\'nski, Wojciech},
TITLE={On conjugacy of maximal abelian subalgebras and the outer automorphism group of the Cuntz algebra},
JOURNAL={Proc. Roy. Soc. Edinburgh},
VOLUME={145 A},
YEAR={2015},
PAGES={269--279},
}

\bib{CKS}{article}{
AUTHOR={Conti, Roberto},
author={Kimberley, J. },
author={Szyma\'nski, Wojciech},
TITLE={More localized automorphisms of the Cuntz algebras},
JOURNAL={Proc. Roy. Soc. Edinburgh (Series 2)},
VOLUME={53},
YEAR={2010},
PAGES={619--631},
}

\bib{CRS}{article}{
AUTHOR={Conti, Roberto},
author={R\o rdam, Mikael },
author={Szyma\'nski, Wojciech},
TITLE={Endomorphisms of $\CO_n$ which preserve the canonical UHF-subalgebra},
JOURNAL={J. Funct. Anal.},
VOLUME={259},
YEAR={2010},
PAGES={602--617},
}

\bib{ConSz}{article}{
AUTHOR={Conti, Roberto},
author={Szyma\'nski, Wojciech},
TITLE={Labeled trees and localized automorphisms of the Cuntz algebras},
JOURNAL={Trans. Amer. Math. Soc.},
VOLUME={363},
YEAR={2011},
NUMBER={11},
PAGES={5847--5870},
}



\bib{CrispLaca}{article}{
    AUTHOR = {Crisp, John},
    author={Laca, Marcelo},
     TITLE = {Boundary quotients and ideals of {T}oeplitz {$C^*$}-algebras of {A}rtin groups},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {242},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {127--156},
      ISSN = {0022-1236},
     %CODEN = {JFUAAW},
  % MRCLASS = {46L55 (06F15 20F60)},
  %MRNUMBER = {2274018 (2007k:46117)},
%MRREVIEWER = {Alain Valette},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2006.08.001}{10.1016/j.jfa.2006.08.001}},
      % URL = ,
}

\bib{Cun}{article}{%MR0467330,
    AUTHOR = {Cuntz, Joachim},
     TITLE = {Simple C*-algebras generated by isometries},
   JOURNAL = {Comm. Math. Phys.},
%  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {57},
      YEAR = {1977},
    NUMBER = {2},
     PAGES = {173--185},
      ISSN = {0010-3616},
%   MRCLASS = {46L05},
%  MRNUMBER = {0467330 (57 \#7189)},
%MRREVIEWER = {E. Stormer},
}

\bib{CuntzQ}{incollection}{
    AUTHOR = {Cuntz, Joachim},
     TITLE = {{$C^*$}-algebras associated with the {$ax+b$}-semigroup over {$\mathbb{N}$}},
 BOOKTITLE = {{$K$}-theory and noncommutative geometry},
    SERIES = {EMS Ser. Congr. Rep.},
     PAGES = {201--215},
 PUBLISHER = {Eur. Math. Soc., Z\"urich},
      YEAR = {2008},
}

\bib{Cuntz-review}{incollection}{
  title={C$^*$-Algebras associated with algebraic actions},
  author={Cuntz, Joachim},
  booktitle={Operator Algebras and Applications},
  pages={145--159},
  year={2016},
  publisher={Springer}
}


\bib{CDL13}{article}{%cuntz2013c,
  title={C\^{}*-algebras of Toeplitz type associated with algebraic number fields},
  author={Cuntz, Joachim},
  author={Deninger, Christopher},
  author={Laca, Marcelo},
  journal={Math. Ann.},
  volume={355},
  number={4},
  pages={1383--1423},
  year={2013},
  publisher={Springer}
}


\bib{CEL}{article}{%MR3094498,
AUTHOR = {Cuntz, Joachim},
AUTHOR = {Echterhoff, Siegfried},
AUTHOR = {Li, Xin},
TITLE = {On the $K$-theory of crossed products by automorphic semigroup actions}, %{$K$}
JOURNAL = {Q. J. Math.},
%FJOURNAL = {The Quarterly Journal of Mathematics},
VOLUME = {64},
YEAR = {2013},
NUMBER = {3},
     PAGES = {747--784},
      ISSN = {0033-5606},
   %MRCLASS = {19Dxx},
  %MRNUMBER = {3094498},
       DOI = {\href{http://dx.doi.org/10.1093/qmath/hat021}{10.1093/qmath/hat021}},
}	

\bib{CEL2}{article}{
	AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Echterhoff, Siegfried},
    AUTHOR = {Li, Xin},
     TITLE = {On the $K$-theory of the C*-algebra generated by the left regular representation of an Ore semigroup}, %{$K$}
   JOURNAL = {J. Eur. Math. Soc. (JEMS)},
  %FJOURNAL = {Journal of the European Mathematical Society (JEMS)},
    VOLUME = {17},
      YEAR = {2015},
    NUMBER = {3},
     PAGES = {645--687},
      ISSN = {1435-9855},
  % MRCLASS = {46L05 (11R04 19K35 22D25)},
 % MRNUMBER = {3323201},
%MRREVIEWER = {\Dbar ỗ Ngọc Diệp},
       DOI = {\href{http://dx.doi.org/10.4171/JEMS/513}{10.4171/JEMS/513}},
%       URL = {http://dx.doi.org/10.4171/JEMS/513},
}	

\bib{CELY}{book}{
    AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Echterhoff, Siegfried},
    author={Li, Xin},
    author={Yu, Guoliang},
     TITLE = {K-Theory for Group $C^*$-Algebras and Semigroup $C^*$-Algebras},
    SERIES = {Oberwolfach Seminars},
 PUBLISHER = {Birkh\"auser Basel},
%   ADDRESS = {},
      YEAR = {2017},
     PAGES = {x+317},
      ISBN = {978-3-319-59914-4},
      ISSN={1661-237X},
  % MRCLASS = {19K35 (46L80)},
 % MRNUMBER = {1124848 (94b:19008)},
%MRREVIEWER = {Jeffrey Fox},
       DOI = {\href{http://www.springer.com/de/book/9783319599144}{10.1007/978-3-319-59915-1}},
}


\bib{CK}{article} {%MR561974,
    AUTHOR = {Cuntz, Joachim}, 
    AUTHOR = {Krieger, Wolfgang},
     TITLE = {A class of C*-algebras and topological {M}arkov chains},
   JOURNAL = {Invent. Math.},
  %FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {56},
      YEAR = {1980},
    NUMBER = {3},
     PAGES = {251--268},
      ISSN = {0020-9910},
     %CODEN = {INVMBH},
   %MRCLASS = {46L55 (54H20 58G10)},
  %MRNUMBER = {561974 (82f:46073a)},
%MRREVIEWER = {R. J. Nagel},
       DOI = {\href{http://dx.doi.org/10.1007/BF01390048}{10.1007/BF01390048}},
}

\bib{CL}{incollection}{%MR2732050,
    AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Li, Xin},
     TITLE = {The regular C*-algebra of an integral domain},
 BOOKTITLE = {Quanta of maths},
    SERIES = {Clay Math. Proc.},
    VOLUME = {11},
     PAGES = {149--170},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2010},
  % MRCLASS = {46L55 (11M55 11R04 46L05)},
 % MRNUMBER = {2732050 (2012c:46173)},
%MRREVIEWER = {Bora Yalkinoglu},
}

\bib{CLintegral2}{article}{
    AUTHOR = {Cuntz, Joachim},
    author={Li, Xin},
     TITLE = {{$C^*$}-algebras associated with integral domains and crossed products by actions on adele spaces},
   JOURNAL = {J. Noncommut. Geom.},
 % FJOURNAL = {Journal of Noncommutative Geometry},
    VOLUME = {5},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {1--37},
      ISSN = {1661-6952},
}

\bib{CuntzVershik}{article}{
		AUTHOR = {Cuntz, Joachim},
		author={Vershik, Anatoly},
     TITLE = {{$C^*$}-algebras associated with endomorphisms and polymorphisms of compact abelian groups},
      YEAR = {2013},
issn={0010-3616},
journal={Comm. Math. Phys.},
volume={321},
number={1},
doi= {\href{http://dx.doi.org/10.1007/s00220-012-1647-0}{10.1007/s00220-012-1647-0}},
publisher={Springer-Verlag},
pages={157-179},
%language={English}
}	

\bib{DE}{book}{%MR2457798,
    AUTHOR = {Deitmar, Anton},
    AUTHOR = {Echterhoff, Siegfried},
     TITLE = {Principles of Harmonic Analysis},
    SERIES = {Universitext},
 PUBLISHER = {Springer, New York},
      YEAR = {2009},
     PAGES = {xvi+333},
      ISBN = {978-0-387-85468-7},
  % MRCLASS = {43-01 (22Dxx 22E30 46J10 46L05)},
 % MRNUMBER = {2457798 (2010g:43001)},
%MRREVIEWER = {Krishnan Parthasarathy},
}

\bib{DFK}{article}{
 	AUTHOR 	= {Davidson, Kenneth R.},
    AUTHOR 	= {Fuller, Adam H.},
    AUTHOR 	= {Kakariadis, Evgenios T.A.},
    TITLE	= {Semicrossed products of operator algebras by semigroups},
    %JOURNAL = {preprint},
    NOTE 	= {preprint \href{http://arxiv.org/abs/1404.1906v1}{arxiv:1404.1906v1}}, 
}

\bib{DG}{article}{%MR2055042,
    AUTHOR = {Duncan, Andrew},
    AUTHOR = {Gilman, Robert H.},
     TITLE = {Word hyperbolic semigroups},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
%  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical Society},
    VOLUME = {136},
      YEAR = {2004},
    NUMBER = {3},
     PAGES = {513--524},
      ISSN = {0305-0041},
%     CODEN = {MPCPCO},
  % MRCLASS = {20M05 (20M35)},
%  MRNUMBER = {2055042 (2004m:20106)},
%MRREVIEWER = {P. M. Higgins},
       DOI = {\href{http://dx.doi.org/10.1017/S0305004103007497}{10.1017/S0305004103007497}},
%       URL = ,
}

\bib{Dykema}{article}{
  author={Dykema, Kenneth J.},
  author={Shlyakhtenko, Dimitri},
  title={Exactness of Cuntz--Pimsner C*-algebras},
  journal={Proceedings of the Edinburgh Mathematical Society (Series 2)},
  volume={44},
  number={02},
  pages={425--444},
  year={2001},
  publisher={Cambridge Univ. Press},
}

\bib{dJST}{article}{%MR2913686,
    AUTHOR = {de Jeu, Marcel},
    AUTHOR = {Svensson, Christian},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {On the {B}anach {$\ast$}-algebra crossed product associated with a topological dynamical system},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {11},
     PAGES = {4746--4765},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46H99 54H20)},
 % MRNUMBER = {2913686},
%MRREVIEWER = {Claire Anantharaman-Delaroche},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2012.03.013}{10.1016/j.jfa.2012.03.013}},
       %URL = ,
}

\bib{dlH}{book}{%MR1786869,
    AUTHOR = {de la Harpe, Pierre},
     TITLE = {Topics in Geometric Group Theory},
    SERIES = {Chicago Lectures in Mathematics},
 PUBLISHER = {University of Chicago Press, Chicago, IL},
      YEAR = {2000},
     PAGES = {vi+310},
      ISBN = {0-226-31719-6; 0-226-31721-8},
  % MRCLASS = {20F65 (20F69 57M07)},
 % MRNUMBER = {1786869 (2001i:20081)},
%MRREVIEWER = {Lee Mosher},
}

\bib{ELR}{article}{%MR3505132,
    AUTHOR = {Eilers, S{\o}ren},
    author={Li, Xin},
    author={Ruiz, Efren},
     TITLE = {The isomorphism problem for semigroup {$C^*$}-algebras of right-angled {A}rtin monoids},
   JOURNAL = {Doc. Math.},
  %FJOURNAL = {Documenta Mathematica},
    VOLUME = {21},
      YEAR = {2016},
     PAGES = {309--343},
      ISSN = {1431-0635},
  % MRCLASS = {46L05 (20M05 46L35)},
 % MRNUMBER = {3505132},
%MRREVIEWER = {Chao You},
}

\bib{EF}{article}{%MR2586349,
    AUTHOR = {Einsiedler, Manfred},
    AUTHOR = {Fish, Alexander},
     TITLE = {Rigidity of measures invariant under the action of a multiplicative semigroup of polynomial growth on $\IT$},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {30},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {151--157},
      ISSN = {0143-3857},
 %  MRCLASS = {37A10 (28D10 37A25)},
 % MRNUMBER = {2586349 (2011a:37005)},
%MRREVIEWER = {A. I. Danilenko},
       DOI = {\href{http://dx.doi.org/10.1017/S014338570800103X}{10.1017/S014338570800103X}},
}

\bib{EK}{article}{%MR2191228,
    AUTHOR = {Einsiedler, Manfred},
    AUTHOR = {Katok, Anatole},
     TITLE = {Rigidity of measures---the high entropy case and non-commuting foliations},
 %     NOTE = {Probability in mathematics},
   JOURNAL = {Israel J. Math.},
%  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {148},
      YEAR = {2005},
     PAGES = {169--238},
      ISSN = {0021-2172},
 %    CODEN = {ISJMAP},
 %  MRCLASS = {37C85 (37A15 37C40 37D30)},
 % MRNUMBER = {2191228 (2007d:37034)},
%MRREVIEWER = {S. G. Dani},
       DOI = {\href{http://dx.doi.org/10.1007/BF02775436}{10.1007/BF02775436}},
%       URL = ,
}

\bib{ER2}{article}{%MR2162134,
    AUTHOR = {Endimioni, G{\'e}rard},
    AUTHOR = {Robinson, Derek J. S.},
     TITLE = {On co-{H}opfian groups},
   JOURNAL = {Publ. Math. Debrecen},
 % FJOURNAL = {Publicationes Mathematicae Debrecen},
    VOLUME = {67},
      YEAR = {2005},
    NUMBER = {3-4},
     PAGES = {423--436},
      ISSN = {0033-3883},
   %  CODEN = {PUMAAR},
  % MRCLASS = {20F99},
 % MRNUMBER = {2162134 (2006e:20082)},
%MRREVIEWER = {Javier Otal},
}

\bib{Evans}{article}{
AUTHOR = {Evans, D. Gwion},
     TITLE = {On the {$K$}-theory of higher rank graph {$C\sp *$}-algebras},
   JOURNAL = {New York J. Math.},
 % FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {14},
      YEAR = {2008},
     PAGES = {1--31},
      ISSN = {1076-9803},
 %  MRCLASS = {46L80 (19K14 46L35 46M18)},
  %MRNUMBER = {2383584 (2009e:46065)},
%MRREVIEWER = {Benton L. Duncan},
       URL = {\href{http://nyjm.albany.edu:8000/j/2008/14_1.html}{nyjm:8000/j/2008/14_1}},
}

\bib{Ex}{article}{
	title={The soft torus and applications to almost commuting matrices},
	author={Exel, R.},
	year={1993},
	journal={Pacific J. Math.},
	volume={160},
	number={2},
	pages={207--217}
}

\bib{Exe1}{article} {%MR2032486,
    AUTHOR = {Exel, Ruy},
     TITLE = {A new look at the crossed-product of a C*-algebra by an endomorphism},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {23},
      YEAR = {2003},
    NUMBER = {6},
     PAGES = {1733--1750},
      ISSN = {0143-3857},
  % MRCLASS = {46L55 (37B10)},
 % MRNUMBER = {2032486 (2004k:46119)},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385702001797}{10.1017/S0143385702001797}},
}

\bib{Exe2}{article}{%MR1966826,
    AUTHOR = {Exel, Ruy},
     TITLE = {Crossed-products by finite index endomorphisms and {KMS} states},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {199},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {153--188},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46L30)},
 % MRNUMBER = {1966826 (2004b:46094)},
%MRREVIEWER = {Masaharu Kusuda},
       DOI = {\href{http://dx.doi.org/10.1016/S0022-1236(02)00023-X}{10.1016/S0022-1236(02)00023-X}},
}

\bib{EaHR}{article} {%MR2985865,
    AUTHOR = {Exel, Ruy},
    AUTHOR = {an Huef, Astrid},
    AUTHOR = {Raeburn, Iain},
     TITLE = {Purely infinite simple {$C^*$}-algebras associated to integer dilation matrices},
   JOURNAL = {Indiana Univ. Math. J.},
 % FJOURNAL = {Indiana University Mathematics Journal},
    VOLUME = {60},
      YEAR = {2011},
    NUMBER = {3},
     PAGES = {1033--1058},
      ISSN = {0022-2518},
%     CODEN = {IUMJAB},
 %  MRCLASS = {46L05 (46L55)},
  %MRNUMBER = {2985865},
%MRREVIEWER = {Xin Li},
       DOI = {\href{http://dx.doi.org/10.1512/iumj.2011.60.4331}{10.1512/iumj.2011.60.4331}},
       %URL = ,
}

\bib{EP}{article}{
    AUTHOR = {Exel, Ruy}, 
    AUTHOR = {Pardo, Enrique},
     TITLE = {The tight groupoid of an inverse semigroup},
DOI = {\href{http://arxiv.org/abs/1408.5278v2}{arxiv:1408.5278v2}},
}

\bib{ER}{article}{%MR2371594,
    AUTHOR = {Exel, Ruy}, 
    AUTHOR = {Renault, Jean},
     TITLE = {Semigroups of local homeomorphisms and interaction groups},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {27},
      YEAR = {2007},
    NUMBER = {6},
     PAGES = {1737--1771},
      ISSN = {0143-3857},
  % MRCLASS = {46L55 (37B05 46L05)},
 % MRNUMBER = {2371594 (2009k:46124)},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385707000193}{10.1017/S0143385707000193}},
}	

\bib{EV}{article} {%MR2195591,
    AUTHOR = {Exel, Ruy},
    AUTHOR = {Vershik, Anatoly},
     TITLE = {C*-algebras of irreversible dynamical systems},
   JOURNAL = {Canad. J. Math.},
%  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
%              Math\'ematiques},
    VOLUME = {58},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {39--63},
      ISSN = {0008-414X},
%     CODEN = {CJMAAB},
%   MRCLASS = {46L55 (37A55 46L05)},
%  MRNUMBER = {2195591 (2007d:46058)},
%MRREVIEWER = {Fr{\'e}d{\'e}ric Latr{\'e}moli{\`e}re},
       DOI = {\href{http://dx.doi.org/10.4153/CJM-2006-003-x}{10.4153/CJM-2006-003-x}},
}


\bib{FPW}{article}{%MR3085824,
    AUTHOR = {Farthing, Cynthia},
    AUTHOR = {Patani, Nura},
    AUTHOR = {Willis, Paulette N.},
     TITLE = {The crossed-product structure of C*-algebras arising from topological dynamical systems},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {70},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {191--210},
      ISSN = {0379-4024},
   %MRCLASS = {46L55 (37A55)},
  %MRNUMBER = {3085824},
       DOI = {\href{http://dx.doi.org/10.7900/jot.2011may31.1924}{10.7900/jot.2011may31.1924}},
}

\bib{Fow1}{article} {%MR1715181,
    AUTHOR = {Fowler, Neal J.},
    TITLE = {Compactly-aligned discrete product systems, and generalization of $\CO_{\infty}$},
   JOURNAL = {Internat. J. Math.},
  %FJOURNAL = {International Journal of Mathematics},
    VOLUME = {10},
      YEAR = {1999},
    NUMBER = {6},
     PAGES = {721--738},
      ISSN = {0129-167X},
  % MRCLASS = {46L05},
 % MRNUMBER = {1715181 (2002f:46104)},
       DOI = {\href{http://dx.doi.org/10.1142/S0129167X99000306}{10.1142/S0129167X99000306}},
}

\bib{Fow2}{article} {%MR1907896,
    AUTHOR = {Fowler, Neal J.},
     TITLE = {Discrete product systems of {H}ilbert bimodules},
   JOURNAL = {Pacific J. Math.},
 % FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {204},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {335--375},
      ISSN = {0030-8730},
%     CODEN = {PJMAAI},
%   MRCLASS = {46L08},
%  MRNUMBER = {1907896 (2003g:46070)},
%MRREVIEWER = {Arup Kumar Pal},
       DOI = {\href{http://dx.doi.org/10.2140/pjm.2002.204.335}{10.2140/pjm.2002.204.335}},
}

\bib{FS}{article}{
AUTHOR = {Fowler, Neal J.},
author={Sims, Aidan},
     TITLE = {Product systems over right-angled {A}rtin semigroups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {354},
      YEAR = {2002},
    NUMBER = {4},
     PAGES = {1487--1509 (electronic)},
      ISSN = {0002-9947},
     %CODEN = {TAMTAM},
   %MRCLASS = {18D10 (18B40 20F36 46L06)},
 % MRNUMBER = {1873016 (2002j:18006)},
%MRREVIEWER = {V{\'a}clav Koubek},
     URL = {\href{http://dx.doi.org/10.1090/S0002-9947-01-02911-7}{$10.1090/S0002-9947-01-02911-7$}},
}

\bib{Fur}{article} {%MR0213508,
    AUTHOR = {Furstenberg, Hillel},
     TITLE = {Disjointness in ergodic theory, minimal sets, and a problem in {D}iophantine approximation},
   JOURNAL = {Math. Systems Theory},
  %FJOURNAL = {Mathematical Systems Theory. An International Journal on
%              Mathematical Computing Theory},
    VOLUME = {1},
      YEAR = {1967},
     PAGES = {1--49},
      ISSN = {0025-5661},
   %MRCLASS = {28.70 (10.00)},
 % MRNUMBER = {0213508 (35 \#4369)},
%MRREVIEWER = {W. Parry}
}


\bib{Ga}{book} {%MR0107648,
    AUTHOR = {Gantmacher, F. R.},
     TITLE = {Applications of the theory of matrices},
    SERIES = {Translated by J. L. Brenner, with the assistance of D. W. Bushaw and S. Evanusa},
 PUBLISHER = {Interscience Publishers, Inc., New York},
      YEAR = {1959},
     PAGES = {ix+317}
  % MRCLASS = {15.00 (65.00)},
 % MRNUMBER = {0107648 (21 \#6372b)},
}

\bib{GG}{incollection}{%MR2962880,
    AUTHOR = {Goldsmith, Brendan},
    AUTHOR = {Gong, Ketao},
     TITLE = {A note on {H}opfian and co-{H}opfian abelian groups},
 BOOKTITLE = {Groups and Model Theory},
    SERIES = {Contemp. Math.},
    VOLUME = {576},
     PAGES = {129--136},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2012},
  % MRCLASS = {20K30 (20K21)},
 % MRNUMBER = {2962880},
%MRREVIEWER = {Simion Sorin P. Breaz},
       DOI = {\href{http://dx.doi.org/10.1090/conm/576/11356}{10.1090/conm/576/11356}},
}

\bib{Gl}{article}{
	AUTHOR = {Glimm, James G.},
	TITLE = {On a cerain class of operator algebras},
	JOURNAL = {Trans. Amer. Math. Soc.},
	VOLUME = {95},
	YEAR = {1960},
	PAGES = {318--340}
}

\bib{Hed}{article}{%MR0259881,
    AUTHOR = {Hedlund, Gustav A.},
     TITLE = {Endomorphisms and automorphisms of the shift dynamical system},
   JOURNAL = {Math. Systems Theory},
%  FJOURNAL = {Mathematical Systems Theory. An International Journal on Mathematical Computing Theory},
    VOLUME = {3},
      YEAR = {1969},
     PAGES = {320--375},
      ISSN = {0025-5661},
  % MRCLASS = {54.82},
 % MRNUMBER = {0259881 (41 \#4510)},
%MRREVIEWER = {W. R. Utz},
}

\bib{hr}{book}{ %MR0156915
   author={Hewitt, Edwin},
   author={Ross, Kenneth A.},
   title={Abstract harmonic analysis. Vol. I: Structure of topological
   groups. Integration theory, group representations},
   series={Die Grundlehren der mathematischen Wissenschaften, Bd. 115},
   publisher={Academic Press, Inc., Publishers, New York; Springer-Verlag,
   Berlin-G\"ottingen-Heidelberg},
   date={1963},
   pages={viii+519},
   review={\MR{0156915 (28 \#158)}},
}

\bib{Hir}{article} {%MR1896827,
    AUTHOR = {Hirshberg, Ilan},
     TITLE = {On $C^*$-algebras associated to certain endomorphisms of discrete groups},
   JOURNAL = {New York J. Math.},
  %FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {8},
      YEAR = {2002},
     PAGES = {99--109 (electronic)},
      ISSN = {1076-9803},
  % MRCLASS = {46L55},
 % MRNUMBER = {1896827 (2003d:46090)},
%MRREVIEWER = {Sriwulan Adji},
       NOTE = {\href{http://nyjm.albany.edu:8000/j/2002/8_99.html}{$nyjm.albany.edu:8000/j/2002/8_99$}},
}

\bib{HLS}{article}{
AUTHOR = {Hong, Jeong Hee},
AUTHOR = {Larsen, Nadia S.},
AUTHOR = {Szyma\'{n}ski, Wojciech},
TITLE  = {KMS states on Nica-Toeplitz algebras of product systems},
journal = {Internat. J. Math.},
volume = {23},
number = {12},
pages = {1250123},
year = {2012},
doi = {\href{http://www.worldscientific.com/doi/abs/10.1142/S0129167X12501236}{10.1142/S0129167X12501236}},
%eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0129167X12501236}
}


\bib{JT}{book} {%MR1124848,
    AUTHOR = {Jensen, Kjeld Knudsen},
    AUTHOR = {Thomsen, Klaus},
     TITLE = {Elements of {$KK$}-Theory},
    SERIES = {Mathematics: Theory \& Applications},
 PUBLISHER = {Birkh\"auser Boston Inc.},
   ADDRESS = {Boston, MA},
      YEAR = {1991},
     PAGES = {viii+202},
      ISBN = {0-8176-3496-7},
  % MRCLASS = {19K35 (46L80)},
 % MRNUMBER = {1124848 (94b:19008)},
%MRREVIEWER = {Jeffrey Fox},
       DOI = {\href{http://dx.doi.org/10.1007/978-1-4612-0449-7}{10.1007/978-1-4612-0449-7}},
}

\bib{KOQ}{article}{ %MR3300223
   author={Kaliszewski, S.},
   author={Omland, Tron},
   author={Quigg, John},
   title={Cuntz-Li algebras from $a$-adic numbers},
   journal={Rev. Roumaine Math. Pures Appl.},
   volume={59},
   date={2014},
   number={3},
   pages={331--370},
   issn={0035-3965},
   review={\MR{3300223}},
}

\bib{kasparov}{article}{
author={Kasparov, Gennadi},
title={{Equivariant {$KK$}-theory and the Novikov conjecture}},
volume={91},
journal={Invent. Math.},
year={1988},
pages={147--201}
}

\bib{KatsuraI}{article} {%MR2067120,
    AUTHOR = {Katsura, Takeshi},
     TITLE = {A class of C*-algebras generalizing both graph algebras and homeomorphism C*-algebras. {I}. {F}undamental results},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {356},
      YEAR = {2004},
    NUMBER = {11},
     PAGES = {4287--4322 (electronic)},
      ISSN = {0002-9947},
    % CODEN = {TAMTAM},
   %MRCLASS = {46L05 (37B99 46L55 46L80)},
 %MRNUMBER = {2067120 (2005b:46119)},
%MRREVIEWER = {Valentin Deaconu},
       DOI = {\href{http://dx.doi.org/10.1090/S0002-9947-04-03636-0}{10.1090/S0002-9947-04-03636-0}},
}

\bib{KatsuraIV}{article}{
    AUTHOR = {Katsura, Takeshi},
     TITLE = {A class of {$C^*$}-algebras generalizing both graph algebras and homeomorphism {$C^*$}-algebras. {IV}. {P}ure infiniteness},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {254},
      YEAR = {2008},
    NUMBER = {5},
     PAGES = {1161--1187},
      ISSN = {0022-1236},
 %    CODEN = {JFUAAW},
}

\bib{Kir}{article}{
	AUTHOR 	= {Kirchberg, Eberhard},
	TITLE	= {The classication of purely infinite C*-algebras using Kasparov's theory},
	JOURNAL = {to appear in Fields Inst. Commun, Amer. Math. Soc. Providence},
}

\bib{KK}{article}{
	AUTHOR = {Kalantar, Mehrdad},
	AUTHOR = {Kennedy, Matthew},
	TITLE  = {Boundaries of reduced C*-algebras of discrete groups},
	JOURNAL = {to appear in J. Reine Angew. Math.},
    NOTE 	= {preprint \href{http://arxiv.org/pdf/1405.4359v1}{arxiv:1405.4359v1}},
}

\bib{KP}{article}{
AUTHOR = {Kumjian, Alex},
author={Pask, David},
     TITLE = {Higher rank graph {$C^*$}-algebras},
   JOURNAL = {New York J. Math.},
%  FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {6},
      YEAR = {2000},
     PAGES = {1--20},
      ISSN = {1076-9803},
   %MRCLASS = {46L35 (46L45)},
  %MRNUMBER = {1745529 (2001b:46102)},
%MRREVIEWER = {Michael Frank},
       URL = {\href{http://nyjm.albany.edu:8000/j/2000/6_1.html}{nyjm:8000/j/2000/6_1}},
}

%\bib{KPRR}{article} {%MR1432596,
 %   AUTHOR = {Kumjian, Alex},
 %   AUTHOR = {Pask, David},
 %   AUTHOR = {Raeburn, Iain},
 %   AUTHOR = {Renault, Jean},
 %    TITLE = {Graphs, groupoids, and {C}untz-{K}rieger algebras},
 %  JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
 %   VOLUME = {144},
 %     YEAR = {1997},
 %   NUMBER = {2},
 %    PAGES = {505--541},
 %     ISSN = {0022-1236},
    % CODEN = {JFUAAW},
  % MRCLASS = {46L05 (46L55)},
 % MRNUMBER = {1432596 (98g:46083)},
%MRREVIEWER = {Masatoshi Enomoto},
  %     DOI = {10.1006/jfan.1996.3001},
  %     URL = {http://dx.doi.org/10.1006/jfan.1996.3001},
%}

\bib{Kri}{article} {%MR1934386,
    AUTHOR = {Kribs, David W.},
     TITLE = {Inductive limit algebras from periodic weighted shifts on {F}ock space},
   JOURNAL = {New York J. Math.},
%  FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {8},
      YEAR = {2002},
     PAGES = {145--159 (electronic)},
      ISSN = {1076-9803},
%   MRCLASS = {46L05 (46L35)},
%  MRNUMBER = {1934386 (2004b:46073)},
%MRREVIEWER = {Il Bong Jung},
       NOTE = {\href{http://nyjm.albany.edu:8000/j/2002/8_145.html}{nyjm.albany.edu:8000/j/2002/8_145}},
}

%\bib{KS}{article}{
%author={Kwa\'{s}niewski, Bartosz},
%author={Szyma\'{n}ski, Wojciech},
%title={Topological aperiodicity for product systems over semigroups of Ore type},
%note={preprint \href{http://arxiv.org/pdf/1312.7472v1}{arxiv:1312.7472v1}},
%}

\bib{KS}{article}{
author={Kadison, Richard V.},
author = {Singer, Isadore M.},
title={{Extensions of pure states}},
year={1959},
journal={{Amer. J. Math.}},
volume={81},
pages={383--400}
}


\bib{KT}{article}{%MR1088230,
    AUTHOR = {Kawamura, Shinz{\=o}},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {Properties of topological dynamical systems and corresponding {$C^*$}-algebras},
   JOURNAL = {Tokyo J. Math.},
%  FJOURNAL = {Tokyo Journal of Mathematics},
    VOLUME = {13},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {251--257},
      ISSN = {0387-3870},
%   MRCLASS = {46L55 (54H20)},
%  MRNUMBER = {1088230 (92e:46131)},
%MRREVIEWER = {John Quigg},
       DOI = {\href{http://dx.doi.org/10.3836/tjm/1270132260}{10.3836/tjm/1270132260}},
 %      URL = ,
}

\bib{Lac}{article}{
    AUTHOR = {Laca, Marcelo},
     TITLE = {From endomorphisms to automorphisms and back: dilations and full corners},
   JOURNAL = {J. London Math. Soc. (2)},
%  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {61},
    YEAR = {2000},
    NUMBER = {3},
    PAGES = {893--904},
    DOI = {\href{http://dx.doi.org/10.1112/S0024610799008492}{10.1112/S0024610799008492}},
}

\bib{LaNe}{article} {%MR2785897,
    AUTHOR = {Laca, Marcelo},
    author={Neshveyev, Sergey},
     TITLE = {Type {$\rm III\sb 1$} equilibrium states of the {T}oeplitz algebra of the affine semigroup over the natural numbers},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {261},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {169--187},
      ISSN = {0022-1236},
     %CODEN = {JFUAAW},
   %MRCLASS = {46L55 (11M55 46L30)},
  %MRNUMBER = {2785897},
%MRREVIEWER = {Douglas R. Farenick},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2011.03.009}{10.1016/j.jfa.2011.03.009}},
  %     URL = {http://dx.doi.org/10.1016/j.jfa.2011.03.009},
}

\bib{LR1}{article}{
AUTHOR = {Laca, Marcelo},
author={Raeburn, Iain},
     TITLE = {Semigroup crossed products and the {T}oeplitz algebras of nonabelian groups},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {139},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {415--440},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46L35 47B35)},
 % MRNUMBER = {1402771 (97h:46109)},
%MRREVIEWER = {Erik B{\'e}dos},
       DOI = {\href{http://dx.doi.org/10.1006/jfan.1996.0091}{10.1006/jfan.1996.0091}},
}

\bib{LR2}{article}{%MR2671177,
    AUTHOR = {Laca, Marcelo},
    author={Raeburn, Iain},
     TITLE = {Phase transition on the {T}oeplitz algebra of the affine semigroup over the natural numbers},
   JOURNAL = {Adv. Math.},
  %FJOURNAL = {Advances in Mathematics},
    VOLUME = {225},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {643--688},
      ISSN = {0001-8708},
     %CODEN = {ADMTA4},
   %MRCLASS = {46L55 (46L30)},
  %MRNUMBER = {2671177 (2012g:46102)},
%MRREVIEWER = {Erik B{\'e}dos},
       DOI = {\href{http://dx.doi.org/10.1016/j.aim.2010.03.007}{10.1016/j.aim.2010.03.007}},
%       URL = {http://dx.doi.org/10.1016/j.aim.2010.03.007},
}

\bib{LRR}{article}{%MR2838037,
    AUTHOR = {Laca, Marcelo},
    AUTHOR = {Raeburn, Iain},
    AUTHOR = {Ramagge, Jacqui},
     TITLE = {Phase transition on {E}xel crossed products associated to dilation matrices},
   JOURNAL = {J. Funct. Anal.},
  %FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {261},
      YEAR = {2011},
    NUMBER = {12},
     PAGES = {3633--3664},
      ISSN = {0022-1236},
     %CODEN = {JFUAAW},
   %MRCLASS = {46L30 (46L55)},
  %MRNUMBER = {2838037},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href {http://dx.doi.org/10.1016/j.jfa.2011.08.015}{10.1016/j.jfa.2011.08.015}},
  %     URL = {http://dx.doi.org/10.1016/j.jfa.2011.08.015},
}

\bib{LRRW}{article}{%MR3192463,
    AUTHOR = {Laca, Marcelo},
    AUTHOR = {Raeburn, Iain},
    AUTHOR = {Ramagge, Jacqui},
    AUTHOR = {Whittaker, Michael F.},
     TITLE = {Equilibrium states on the {C}untz-{P}imsner algebras of self-similar actions},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {266},
      YEAR = {2014},
    NUMBER = {11},
     PAGES = {6619--6661},
      ISSN = {0022-1236},
%   MRCLASS = {46L30 (46L55)},
 % MRNUMBER = {3192463},
%MRREVIEWER = {Mark Tomforde},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2014.03.003}{10.1016/j.jfa.2014.03.003}},
     %  URL = {http://dx.doi.org/10.1016/j.jfa.2014.03.003},
}

\bib{Lan}{book}{%MR1325694,
    AUTHOR = {Lance, Christopher E.},
     TITLE = {Hilbert C*-Modules},
    SERIES = {London Mathematical Society Lecture Note Series},
    VOLUME = {210},
   %   NOTE = {A Toolkit for Operator Algebraists},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1995},
     PAGES = {x+130},
      ISBN = {0-521-47910-X},
  % MRCLASS = {46L05 (46H25 46K05 46L80 46M05 47D25)},
 % MRNUMBER = {1325694 (96k:46100)},
%MRREVIEWER = {Robert S. Doran},
       DOI = {\href{http://dx.doi.org/10.1017/CBO9780511526206}{10.1017/CBO9780511526206}},
}

\bib{Lar}{article} {%MR2669415,
    AUTHOR = {Larsen, Nadia S.},
     TITLE = {Crossed products by abelian semigroups via transfer operators},
   JOURNAL = {Ergodic Theory Dynam. Systems},
%  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {30},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {1147--1164},
      ISSN = {0143-3857},
%   MRCLASS = {46L55},
%  MRNUMBER = {2669415 (2011j:46114)},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385709000509}{10.1017/S0143385709000509}},
}

\bib{LarsenLi}{article}{
    AUTHOR = {Larsen, Nadia S.},
    author = {Li, Xin},
     TITLE = {The $2$-adic ring {$C^*$}-algebra of the integers and its representations},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {4},
     PAGES = {1392--1426},
}

\bib{LR}{article} {%MR2339372,
    AUTHOR = {Larsen, Nadia S.},
    AUTHOR = {Raeburn, Iain},
     TITLE = {Projective multi-resolution analyses arising from direct limits of {H}ilbert modules},
   JOURNAL = {Math. Scand.},
%  FJOURNAL = {Mathematica Scandinavica},
    VOLUME = {100},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {317--360},
      ISSN = {0025-5521},
%     CODEN = {MTSCAN},
%   MRCLASS = {42C40 (28A80 46C05 46H25 46L08 60D05)},
%  MRNUMBER = {2339372 (2008m:42059)},
%MRREVIEWER = {Palle E. T. Jorgensen},
}

\bib{Law1}{article}{%MR2395198,
    AUTHOR = {Lawson, Mark V.},
     TITLE = {A correspondence between a class of monoids and self-similar group actions. {I}},
   JOURNAL = {Semigroup Forum},
  %FJOURNAL = {Semigroup Forum},
    VOLUME = {76},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {489--517},
      ISSN = {0037-1912},
     %CODEN = {SMGFAN},
   %MRCLASS = {20M20 (20M18)},
  %MRNUMBER = {2395198},
%MRREVIEWER = {P. M. Higgins},
       DOI = {\href{http://dx.doi.org/10.1007/s00233-008-9052-x}{10.1007/s00233-008-9052-x}},
  %     URL = {http://dx.doi.org/10.1007/s00233-008-9052-x},
}


\bib{LR17}{article}{%li2017cartan,
  author={Li, Xin},
  author={Renault, Jean},
  title={Cartan subalgebras in C$^*$-algebras. Existence and uniqueness},
  journal={preprint, arXiv:1703.10505},
  year={2017},
}

\bib{Li0}{article}{%MR2721644,
    AUTHOR = {Li, Xin},
     TITLE = {Ring C$^*$-algebras},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {348},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {859--898},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L05 (11R56 16D30 58B34)},
 % MRNUMBER = {2721644 (2012a:46100)},
%MRREVIEWER = {Nadia S. Larsen},
       DOI = {\href{http://dx.doi.org/10.1007/s00208-010-0502-x}{10.1007/s00208-010-0502-x}},
}

\bib{Li1}{article} {%MR2900468,
    AUTHOR = {Li, Xin},
     TITLE = {Semigroup {$C^*$}-algebras and amenability of semigroups},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {10},
     PAGES = {4302--4340},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L05},
%  MRNUMBER = {2900468},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2012.02.020}{10.1016/j.jfa.2012.02.020}},
}

\bib{Li2}{article}{%MR3077884,
    AUTHOR = {Li, Xin},
     TITLE = {Nuclearity of semigroup C*-algebras and the connection to amenability},
   JOURNAL = {Adv. Math.},
%  FJOURNAL = {Advances in Mathematics},
    VOLUME = {244},
      YEAR = {2013},
     PAGES = {626--662},
      ISSN = {0001-8708},
%   MRCLASS = {46L05 (20M12 43A07)},
%  MRNUMBER = {3077884},
%MRREVIEWER = {Takahiro Sudo},
       DOI = {\href{http://dx.doi.org/10.1016/j.aim.2013.05.016}{10.1016/j.aim.2013.05.016}},
}

\bib{LN2}{article}{
    author = {Li, Xin},
    author={Norling, Magnus},
    title  = {Independent resolutions for totally disconnected dynamical systems. {II}. {$C^*$}-algebraic case},
    journal={J. Op. Th.},
    volume={75},
    number={1},
    year={2016},
    pages={163--193},
   doi={\href{http://www.mathjournals.org/jot/2016-075-001/2016-075-001-009.html}{10.7900/jot.2014dec22.2061}},
}
%
%\bib{LR17}{article}{%li2017cartan,
%  title={Cartan subalgebras in C$^*$-algebras. Existence and uniqueness},
%  author={Li, Xin},
%  author={Renault, Jean},
%  journal={preprint, arXiv:1703.10505},
%  year={2017},
%}

\bib{Lin}{article}{%MR1814969,
    AUTHOR = {Lin, Huaxin},
     TITLE = {Classification of simple tracially {AF} C*-algebras},
   JOURNAL = {Canad. J. Math.},
%  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de Math\'{e}matiques},
    VOLUME = {53},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {161--194},
      ISSN = {0008-414X},
   %  CODEN = {CJMAAB},
  % MRCLASS = {46L35 (19K14 46L05 46L80)},
 % MRNUMBER = {1814969 (2002h:46102)},
%MRREVIEWER = {Judith A. Packer},
       DOI = {\href{http://dx.doi.org/10.4153/CJM-2001-007-8}{10.4153/CJM-2001-007-8}},
}

\bib{LS}{incollection} {%MR1928527,
    AUTHOR = {Lind, Douglas},
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Symbolic and algebraic dynamical systems},
 BOOKTITLE = {Handbook of dynamical systems, {V}ol.\ 1{A}},
     PAGES = {765--812},
 PUBLISHER = {North-Holland, Amsterdam},
      YEAR = {2002},
   %MRCLASS = {37B50 (37A15 37B10)},
  %MRNUMBER = {1928527 (2003h:37017)},
%MRREVIEWER = {Anthony Quas},
       DOI = {\href{http://dx.doi.org/10.1016/S1874-575X(02)80012-1}{10.1016/S1874-575X(02)80012-1}},
 %      URL = ,
}


\bib{massey1}{article}{
author={Massey, W. S.},
title={{Exact couples in algebraic topology (Parts I \& II)}},
year={1952},
journal={Ann. Math.},
volume={56},
pages={363--396}
}

\bib{massey2}{article}{
author={Massey, W. S.},
title={{Exact couples in algebraic topology (Parts III, IV \& V)}},
year={1953},
journal={Ann. Math.},
volume={57},
pages={248--286}
}

\bib{Mat}{article} {%MR1774695,
    AUTHOR = {Matsumoto, Kengo},
     TITLE = {On automorphisms of C*-algebras associated with subshifts},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {44},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {91--112},
      ISSN = {0379-4024}
  % MRCLASS = {46L55 (37A55 37B10)},
 % MRNUMBER = {1774695 (2001g:46147)},
%MRREVIEWER = {A. I. Danilenko},
}

\bib{MS}{article}{
	AUTHOR 	= {Matui, Hiroki},
	AUTHOR 	= {Sato, Yasuhiko},
	TITLE 	= {Decomposition rank of UHF-absorbing C*-algebras},
	JOURNAL	= {Duke Math. J.},
	DOI = {\href{http://dx.doi.org/10.1215/00127094-2826908}{10.1215/00127094-2826908}},
%journal = {Duke Mathematical Journal},
%month = {11},
	pages = {2687--2708},
	volume = {163},
	number = {14},
	year = {2014},
}

\bib{MW}{article}{
	AUTHOR 	= {Maloney, Ben},
	AUTHOR 	= {Willis, Paulette N.},
	TITLE 	= {Examples of $*$-commuting maps},
	%JOURNAL	= {preprint},
    NOTE 	= {preprint \href{http://arxiv.org/abs/1101.3795v2}{arxiv:1101.3795v2}},	
}

\bib{Muc}{article}{%MR2136018,
    AUTHOR = {Muchnik, Roman},
     TITLE = {Semigroup actions on $\IT^n$},
   JOURNAL = {Geom. Dedicata},
  %FJOURNAL = {Geometriae Dedicata},
    VOLUME = {110},
      YEAR = {2005},
     PAGES = {1--47},
      ISSN = {0046-5755},
   %  CODEN = {GEMDAT},
  % MRCLASS = {37B05 (20M20)},
 % MRNUMBER = {2136018 (2006i:37022)},
%MRREVIEWER = {Daniel Berend},
}

\bib{Neu}{article}{%MR0062122,
    AUTHOR = {Neumann, B. H.},
     TITLE = {Groups covered by permutable subsets},
   JOURNAL = {J. London Math. Soc.},
  %FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {29},
      YEAR = {1954},
     PAGES = {236--248},
      ISSN = {0024-6107},
   %MRCLASS = {20.0X},
  %MRNUMBER = {0062122 (15,931b)},
%MRREVIEWER = {D. G. Higman},
}

\bib{Nic}{article}{%MR1241114,
    AUTHOR = {Nica, Alexandru},
     TITLE = {C*-algebras generated by isometries and {W}iener-{H}opf operators},
   JOURNAL = {J. Operator Theory},
 % FJOURNAL = {Journal of Operator Theory},
    VOLUME = {27},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {17--52},
      ISSN = {0379-4024},
  % MRCLASS = {46L35 (47B35 47C10)},
 % MRNUMBER = {1241114 (94m:46094)},
%MRREVIEWER = {Ra{\'u}l E. Curto},
}


\bib{NS}{book} {%MR2251116,				%%%notwendig? Walters als Referenz!
    AUTHOR = {Neshveyev, Sergey},
    AUTHOR = {St{\o}rmer, Erling},
     TITLE = {Dynamical Entropy in Operator Algebras},
    SERIES = {Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A Series of Modern Surveys in Mathematics [Results in Mathematics and Related Areas. 3rd Series. A Series of Modern Surveys in Mathematics]},
    VOLUME = {50},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2006},
     PAGES = {x+296},
      ISBN = {978-3-540-34670-8; 3-540-34670-8}
   %MRCLASS = {46L55 (28D20 37B40 46L54 82C10)},
  %MRNUMBER = {2251116 (2007m:46108)},
%MRREVIEWER = {Adam G. Skalski}
}

\bib{Nor1}{article}{%MR3200323,
    AUTHOR = {Norling, Magnus Dahler},
     TITLE = {Inverse semigroup {$C\sp *$}-algebras associated with left cancellative semigroups},
   JOURNAL = {Proc. Edinb. Math. Soc. (2)},
  %FJOURNAL = {Proceedings of the Edinburgh Mathematical Society. Series II},
    VOLUME = {57},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {533--564},
      ISSN = {0013-0915},
%   MRCLASS = {46L05 (06F15 20M18 43A07)},
%  MRNUMBER = {3200323},
%MRREVIEWER = {Camillo Trapani},
       DOI = {\href{http://dx.doi.org/10.1017/S0013091513000540}{10.1017/S0013091513000540}},
%       URL = {http://dx.doi.org/10.1017/S0013091513000540},
}


\bib{olesenPedersen}{article}{
author={Olesen, D.},
author={Pedersen, G. K.},
title={{Partially Inner {$C^{*}$}-dynamical Systems}},
year={1986},
journal={J. Funct. Anal.},
volume={66},
number={2},
pages={262--281}
}

\bib{Oml}{incollection}{%MR3142039,
    AUTHOR = {Omland, Tron},
     TITLE = {{$C\sp *$}-algebras associated with {$a$}-adic numbers},
 BOOKTITLE = {Operator algebra and dynamics},
    SERIES = {Springer Proc. Math. Stat.},
    VOLUME = {58},
     PAGES = {223--238},
 PUBLISHER = {Springer, Heidelberg},
      YEAR = {2013},
   %MRCLASS = {46L55 (11S82)},
  %MRNUMBER = {3142039},
%MRREVIEWER = {Marius V. Ionescu},
       DOI = {\href{http://dx.doi.org/10.1007/978-3-642-39459-1_11}{$10.1007/978-3-642-39459-1_11$}},
     %  URL = ,
}

\bib{Orf}{article} {%MR2550195,
    AUTHOR = {Orfanos, Stefanos},
     TITLE = {Generalized {B}unce-{D}eddens algebras},
   JOURNAL = {Proc. Amer. Math. Soc.},
%  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {138},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {299--308},
      ISSN = {0002-9939},
%     CODEN = {PAMYAR},
%   MRCLASS = {46L55 (46L05 47L65)},
%  MRNUMBER = {2550195 (2011a:46104)},
%MRREVIEWER = {Michal Zajac},
       DOI = {\href{http://dx.doi.org/10.1090/S0002-9939-09-10071-0}{10.1090/S0002-9939-09-10071-0}},
}

\bib{Oza}{article}{%MR1763912,
    AUTHOR = {Ozawa, Narutaka},
     TITLE = {Amenable actions and exactness for discrete groups},
   JOURNAL = {C. R. Acad. Sci. Paris S\'{e}r. I Math.},
%  FJOURNAL = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I.Math\'ematique},
    VOLUME = {330},
      YEAR = {2000},
    NUMBER = {8},
     PAGES = {691--695},
      ISSN = {0764-4442},
   %  CODEN = {CASMEI},
  % MRCLASS = {22D25 (43A35 46L06 46L55)},
 % MRNUMBER = {1763912 (2001g:22007)},
%MRREVIEWER = {Alain Valette},
       DOI = {\href{http://dx.doi.org/10.1016/S0764-4442(00)00248-2}{10.1016/S0764-4442(00)00248-2}},
}

\bib{Par}{incollection}{%MR1411219,
    AUTHOR = {Parry, William},
     TITLE = {Squaring and cubing the circle \mdash {R}udolph's theorem},
 BOOKTITLE = {Ergodic theory of $\Z^d$-actions ({W}arwick,
              1993--1994)},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {228},
     PAGES = {177--183},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {1996},
  % MRCLASS = {28D15 (11K16)},
 % MRNUMBER = {1411219 (97h:28009)},
%MRREVIEWER = {Thomas Ward},
       DOI = {\href{http://dx.doi.org/10.1017/CBO9780511662812.006}{10.1017/CBO9780511662812.006}},
}

\bib{Phi}{article} {%MR1745197,
    AUTHOR = {Phillips, Christopher N.},
     TITLE = {A classification theorem for nuclear purely infinite simple C*-algebras},
   JOURNAL = {Doc. Math.},
  %FJOURNAL = {Documenta Mathematica},
    VOLUME = {5},
      YEAR = {2000},
     PAGES = {49--114 (electronic)},
      ISSN = {1431-0635},
 %  MRCLASS = {46L05 (19K56 46L35 46L80)},
  %MRNUMBER = {1745197 (2001d:46086b)},
%MRREVIEWER = {Mikael R{\o}rdam},
}

\bib{Pim}{incollection} {%MR1426840,
    AUTHOR = {Pimsner, Mihai V.},
     TITLE = {A class of C*-algebras generalizing both {C}untz-{K}rieger algebras and crossed products by $\Z$},
 BOOKTITLE = {Free probability theory ({W}aterloo, {ON}, 1995)},
    SERIES = {Fields Inst. Commun.},
    VOLUME = {12},
     PAGES = {189--212},
 PUBLISHER = {Amer. Math. Soc.},
   ADDRESS = {Providence, RI},
      YEAR = {1997},
  % MRCLASS = {46L05 (46L55 46L80)},
 % MRNUMBER = {1426840 (97k:46069)},
%MRREVIEWER = {Michael Frank},
}

\bib{PV}{article}{
	Author = {Pimsner, Mihai V.},
	Author = {Voiculescu, Dan-Virgil},
	TITLE = {Exact sequences for $K$-groups and Ext-groups of certain cross-product $C^*$-algebras},
	JOURNAL = {J. Operator Theory},
	VOLUME = {4},
	NUMBER = {1},
	YEAR = {1980},
	PAGES = {93--118},
}

\bib{PR}{article} {%MR1964302,
    AUTHOR = {Packer, Judith A.},
    AUTHOR = {Rieffel, Marc A.},
     TITLE = {Wavelet filter functions, the matrix completion problem, and modules over $C(\IT^n)$},
   JOURNAL = {J. Fourier Anal. Appl.},
  %FJOURNAL = {The Journal of Fourier Analysis and Applications},
    VOLUME = {9},
      YEAR = {2003},
    NUMBER = {2},
     PAGES = {101--116},
      ISSN = {1069-5869},
  % MRCLASS = {42C40 (46H25 46L99 94A12)},
 % MRNUMBER = {1964302 (2003m:42063)},
%MRREVIEWER = {Jo Ward},
       DOI = {\href{http://dx.doi.org/10.1007/s00041-003-0010-4}{10.1007/s00041-003-0010-4}},
}


%Referenz im Ausblick zu den Bereichen, die helfen k�nnten. 
\bib{Ren0}{book} {%MR584266,
    AUTHOR = {Renault, Jean},
     TITLE = {A groupoid approach to {$C\sp{\ast} $}-algebras},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {793},
 PUBLISHER = {Springer},
%   ADDRESS = {Berlin},
      YEAR = {1980},
     PAGES = {ii+160},
%      ISBN = {3-540-09977-8},
  % MRCLASS = {46Lxx (22D25 22D40)},
  %MRNUMBER = {584266 (82h:46075)},
%MRREVIEWER = {A. K. Seda},
}

\bib{Ren}{article}{%MR2460017,
    AUTHOR = {Renault, Jean},
     TITLE = {Cartan subalgebras in {$C^*$}-algebras},
   JOURNAL = {Irish Math. Soc. Bull.},
  %FJOURNAL = {Irish Mathematical Society Bulletin},
    NUMBER = {61},
      YEAR = {2008},
     PAGES = {29--63},
      ISSN = {0791-5578},
   %MRCLASS = {46L85 (37B99)},
  %MRNUMBER = {2460017},
%MRREVIEWER = {Benton L. Duncan},
}

\bib{RS}{article}{
	AUTHOR = {Raeburn, Iain},
	AUTHOR = {Szyma{\'n}ski, Wojciech}
	TITLE = {Cuntz-Krieger algebras of infinite graphs and matrices},
	JOURNAL = {Trans. Amer. Math. Soc.},
	VOLUME = {356},
	NUMBER = {1},
	PAGES = {39--59},
	YEAR = {2004},
}

\bib{rordam}{article}{
    AUTHOR = {R{\o}rdam, Mikael},
     TITLE = {Classification of certain infinite simple {$C^*$}-algebras},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {131},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {415--458},
      ISSN = {0022-1236},
     %CODEN = {JFUAAW},
   %MRCLASS = {46L05 (19K35 46L35 46L80)},
 % MRNUMBER = {1345038 (96e:46080a)},
%MRREVIEWER = {Judith A. Packer},
       DOI = {\href{http://dx.doi.org/10.1006/jfan.1995.1095}{10.1006/jfan.1995.1095}},
%       URL = ,
}

\bib{Rud}{article} {%MR1062766,
    AUTHOR = {Rudolph, Daniel J.},
     TITLE = {{$\times 2$} and {$\times 3$} invariant measures and entropy},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  %FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {10},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {395--406},
      ISSN = {0143-3857},
  % MRCLASS = {28D20},
  %MRNUMBER = {1062766 (91g:28026)},
%MRREVIEWER = {Ladislav Andrey},
      DOI = {\href{http://dx.doi.org/10.1017/S0143385700005629}{10.1017/S0143385700005629}},
}

%\bib{RL}{book} {%MR1783408,
 %   AUTHOR = {R{\o}rdam, M.},
  %  AUTHOR = {Larsen, F.},
   % AUTHOR = {Laustsen, N.},
    % TITLE = {An introduction to {$K$}-theory for C*-algebras},
    %SERIES = {London Mathematical Society Student Texts},
    %VOLUME = {49},
 %PUBLISHER = {Cambridge University Press},
 %  ADDRESS = {Cambridge},
  %    YEAR = {2000},
   %  PAGES = {xii+242},
    %  ISBN = {0-521-78334-8; 0-521-78944-3}
  % MRCLASS = {46-01 (19K35 46L80)},
 % MRNUMBER = {1783408 (2001g:46001)},
%MRREVIEWER = {{\'E}ric Leichtnam},
%}


%\bib{RS}{article} {%MR1713322,
 %   AUTHOR = {Robertson, Guyan},
  %  AUTHOR = {Steger, Tim},
   %  TITLE = {Affine buildings, tiling systems and higher rank
    %          {C}untz-{K}rieger algebras},
   %JOURNAL = {J. Reine Angew. Math.},
  %FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik},
    %VOLUME = {513},
     % YEAR = {1999},
     %PAGES = {115--144},
     % ISSN = {0075-4102},
   %  CODEN = {JRMAA8},
  % MRCLASS = {46L05 (20E42 46L55)},
 % MRNUMBER = {1713322 (2000j:46109)},
%MRREVIEWER = {Claudia Pinzari},
      % DOI = {10.1515/crll.1999.057},
       %URL = {http://dx.doi.org/10.1515/crll.1999.057}
%}

\bib{savinienBellissard}{article}{
author={Savinien, J.},
author = {Bellissard, J.},
title={{A spectral sequence for the {$K$}-theory of tiling spaces}},
year={2009},
journal={{Ergod. Th. \& Dynam. Sys.}},
volume={29},
pages={997--1031}
}

\bib{Sch1}{book} {%MR3024809,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Dynamical systems of algebraic origin},
    SERIES = {Modern Birkh\"auser Classics},
%      NOTE = {[2011 reprint of the 1995 original]},% [MR1345152]},
 PUBLISHER = {Birkh\"auser/Springer Basel AG, Basel},
      YEAR = {1995},
     PAGES = {xviii+310},
      ISBN = {978-3-0348-0276-5; 978-3-0348-0277-2},
   %MRCLASS = {01A75},
 % MRNUMBER = {3024809},
}

\bib{Sch2}{incollection} {%MR1905342,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {The dynamics of algebraic {$\Z^d$}-actions},
 BOOKTITLE = {European {C}ongress of {M}athematics, {V}ol. {I} ({B}arcelona,
              2000)},
    SERIES = {Progr. Math.},
    VOLUME = {201},
     PAGES = {543--553},
 PUBLISHER = {Birkh\"auser, Basel},
      YEAR = {2001},
   %MRCLASS = {37A15 (28D20)},
  %MRNUMBER = {1905342 (2003e:37007)},
%MRREVIEWER = {Thomas Ward},
}

\bib{schochet}{article}{
author={Schochet, C.},
title={{Topological methods for {$C^*$}-algebras I: Spectral sequences}},
year={1981},
journal={Pacific J. Math.},
volume={96},
number={1},
pages={193--211},
}

\bib{Sie}{article}{%MR2775364,
    AUTHOR = {Sierakowski, Adam},
     TITLE = {The ideal structure of reduced crossed products},
   JOURNAL = {M\"unster J. Math.},
  %FJOURNAL = {M\"unster Journal of Mathematics},
    VOLUME = {3},
      YEAR = {2010},
     PAGES = {237--261},
      ISSN = {1867-5778},
  % MRCLASS = {46L55 (22D25)},
 % MRNUMBER = {2775364 (2012g:46103)},
%MRREVIEWER = {Tomoyoshi Ohwada},
}


%\bib{Sim}{article} {%MR2270926,
 %   AUTHOR = {Sims, Aidan},
  %   TITLE = {Gauge-invariant ideals in the {$C\sp *$}-algebras of finitely
   %           aligned higher-rank graphs},
   %JOURNAL = {Canad. J. Math.},
  %FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
%              Math\'ematiques},
%    VOLUME = {58},
 %     YEAR = {2006},
  %  NUMBER = {6},
   %  PAGES = {1268--1290},
    %  ISSN = {0008-414X},
   %  CODEN = {CJMAAB},
   %MRCLASS = {46L05},
  %MRNUMBER = {2270926 (2007j:46095)},
%MRREVIEWER = {Bernhard Burgstaller},
     %  URL = {http://journals.cms.math.ca/ams/ams-redirect.php?Journal=CJM&Volume=58&FirstPage=1268}
%}

\bib{Sch3}{incollection} {%MR2090771,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Algebraic $\Z^d$-actions on zero-dimensional compact abelian groups},
 BOOKTITLE = {Modern dynamical systems and applications},
     PAGES = {185--209},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {2004},
  % MRCLASS = {37A15 (28D15 34A45 37A25 37A35)},
 % MRNUMBER = {2090771 (2005g:37003)},
%MRREVIEWER = {Manfred Einsiedler},
}

\bib{Sol}{article}{%MR2225464,
    AUTHOR = {Solel, Baruch},
     TITLE = {Representations of product systems over semigroups and dilations of commuting {CP} maps},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {235},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {593--618},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L08 (46L57 47A20)},
%  MRNUMBER = {2225464 (2007h:46073)},
%MRREVIEWER = {B. V. Rajarama Bhat},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2005.11.014}{10.1016/j.jfa.2005.11.014}},
}

\bib{Spi1}{article}{%MR3000828,
    AUTHOR = {Spielberg, Jack},
     TITLE = {{$C\sp \ast$}-algebras for categories of paths associated to the {B}aumslag-{S}olitar groups},
   JOURNAL = {J. Lond. Math. Soc. (2)},
  %FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {86},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {728--754},
      ISSN = {0024-6107},
   %MRCLASS = {46L05 (46L55 46L80)},
  %MRNUMBER = {3000828},
%MRREVIEWER = {Mark Tomforde},
       DOI = {\href{http://dx.doi.org/10.1112/jlms/jds025}{10.1112/jlms/jds025}},
       %URL = {http://dx.doi.org/10.1112/jlms/jds025},
}

\bib{Stac}{article}{%MR1200792,
    AUTHOR = {Stacey, Peter J.},
     TITLE = {Crossed products of C*-algebras by {$\ast$}-endomorphisms},
   JOURNAL = {J. Austral. Math. Soc. Ser. A},
  %FJOURNAL = {Australian Mathematical Society. Journal. Series A. Pure Mathematics and Statistics},
    VOLUME = {54},
      YEAR = {1993},
    NUMBER = {2},
     PAGES = {204--212},
      ISSN = {0263-6115},
   %  CODEN = {JAMADS},
  % MRCLASS = {46L05 (46L55)},
 % MRNUMBER = {1200792 (94a:46077)},
%MRREVIEWER = {Shuang Zhang},
}


\bib{Sta2}{article}{
	AUTHOR={Stammeier, Nicolai},
	TITLE={Topological freeness for $*$-commuting covering maps},
	journal={to appear in Houston J. Math.},
	NOTE={\href{http://arxiv.org/abs/1311.0793}{arxiv:1311.0793}},
}

\bib{Sta1}{article}{
AUTHOR={Stammeier, Nicolai},
TITLE={On $C^*$-algebras of irreversible algebraic dynamical systems},
journal={J. Funct. Anal.},
%FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {269},
      YEAR = {2015},
    NUMBER = {4},
     PAGES = {1136--1179},
      %ISSN = {0022-1236},
   %MRCLASS = {46L55 (37A55)},
  %MRNUMBER = {3352767},
%MRREVIEWER = {Xin Li},
doi={\href{http://dx.doi.org/10.1016/j.jfa.2015.02.005}{10.1016/j.jfa.2015.02.005}},
 %     URL = {http://dx.doi.org/10.1016/j.jfa.2015.02.005},
}

\bib{Sta3}{article}{
	AUTHOR={Stammeier, Nicolai},
	TITLE={A boundary quotient diagram for right LCM semigroups},
	journal={Semigroup Forum},
	year={2017},
	pages={1--16},
	%issn={1432-2137},
	DOI = {\href{http://dx.doi.org/10.1007/s00233-017-9850-0}{10.1007/s00233-017-9850-0}},
}

\bib{Star}{article}{
author={Starling, Charles},
label={Star15},
title={Boundary quotients of $C^*$-algebras of right LCM semigroups},
journal={J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {268},
      YEAR = {2015},
    NUMBER = {11},
     PAGES = {3326--3356},
   %   ISSN = {0022-1236},
%   MRCLASS = {46L35},
 % MRNUMBER = {3336727},
%MRREVIEWER = {Camillo Trapani},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2015.01.001}{10.1016/j.jfa.2015.01.001}},
%       URL = {http://dx.doi.org/10.1016/j.jfa.2015.01.001},
}

\bib{ST}{article}{%MR2498769,
    AUTHOR = {Svensson, Christian},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {On the commutant of {$C(X)$} in {$C^*$}-crossed products by {$\Z$} and their representations},
   JOURNAL = {J. Funct. Anal.},
  %FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {256},
      YEAR = {2009},
    NUMBER = {7},
     PAGES = {2367--2386},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55},
 % MRNUMBER = {2498769 (2010f:46105)},
%MRREVIEWER = {Steven P. Kaliszewski},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2009.02.002}{10.1016/j.jfa.2009.02.002}},
       %URL = ,
}

\bib{SY}{article} {%MR2718947,
    AUTHOR = {Sims, Aidan},
    AUTHOR = {Yeend, Trent},
     TITLE = {C*-algebras associated to product systems of {H}ilbert bimodules},
   JOURNAL = {J. Operator Theory},
%  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {64},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {349--376},
      ISSN = {0379-4024},
%   MRCLASS = {46L05 (46L08)},
%  MRNUMBER = {2718947 (2011j:46092)},
%MRREVIEWER = {Vladimir Manuilov},
}

%\bib{SZ}{article} {%MR2383707,
 %   AUTHOR = {Skalski, Adam},
  %  AUTHOR = {Zacharias, Joachim},
  %   TITLE = {Entropy of shifts on higher-rank graph {$C\sp *$}-algebras},
  % JOURNAL = {Houston J. Math.},
  %FJOURNAL = {Houston Journal of Mathematics},
   % VOLUME = {34},
    %  YEAR = {2008},
    %NUMBER = {1},
    % PAGES = {269--282},
    %  ISSN = {0362-1588},
    % CODEN = {HJMADZ},
   %MRCLASS = {46L55 (37B10 37B40)},
 % MRNUMBER = {2383707 (2009j:46165)},
%MRREVIEWER = {Aidan D. Sims}
%}

\bib{Zach}{article}{%zacharias2000quasi,
  title={Quasi-free automorphisms of Cuntz-Krieger-Pimsner algebras},
  author={Zacharias, Joachim},
  booktitle={C*-Algebras},
  pages={262--272},
  year={2000},
  publisher={Springer},
}

\bib{takai}{article}{
  title={{On a duality for crossed products by  {$C^*$}-algebras}},
  author={Takai, H.},
  journal={J. Funct. Anal.},
volume={19},
  year={1975},
  pages={25--39},
}

\bib{Tu}{article} {%MR1703305,
    AUTHOR = {Tu, Jean-Louis},
     TITLE = {La conjecture de {B}aum-{C}onnes pour les feuilletages moyennables},
   JOURNAL = {$K$-Theory},
 % FJOURNAL = {$K$-Theory. An Interdisciplinary Journal for the Development,
  %            Application, and Influence of $K$-Theory in the Mathematical
   %           Sciences},
    VOLUME = {17},
      YEAR = {1999},
    NUMBER = {3},
     PAGES = {215--264},
      ISSN = {0920-3036},
   %  CODEN = {KTHEEO},
  % MRCLASS = {19K35 (46L85 58J22)},
 % MRNUMBER = {1703305 (2000g:19004)},
%MRREVIEWER = {Hiroshi Takai},
       DOI = {\href{http://dx.doi.org/10.1023/A:1007744304422}{10.1023/A:1007744304422}},
}

\bib{Vie}{thesis}{
	AUTHOR = {Vieira, Felipe},
	TITLE  = {C*-algebras associated with endomorphisms of groups},
	SCHOOL = {University of M\"unster},
	YEAR   = {2013}, 
	NOTE    = {summary available as \href{http://arxiv.org/pdf/1308.1386v2}{arxiv:1308.1386v2}},
}

\bib{Wal}{book}{%MR648108,
    AUTHOR = {Walters, Peter},
     TITLE = {An Introduction to Ergodic Theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {79},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {1982},
     PAGES = {ix+250},
      ISBN = {0-387-90599-5},
   %MRCLASS = {28Dxx (54H20 58F11)},
  %MRNUMBER = {648108 (84e:28017)},
%MRREVIEWER = {M. A. Akcoglu},
}
% , and Isadore M. 

\bib{Wat}{article}{%MR996807,
    AUTHOR = {Watatani, Yasuo},
     TITLE = {Index for C*-subalgebras},
   JOURNAL = {Mem. Amer. Math. Soc.},
 % FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {83},
      YEAR = {1990},
    NUMBER = {424},
     PAGES = {vi+117},
      ISSN = {0065-9266},
   %  CODEN = {MAMCAU},
%   MRCLASS = {46L05 (19K14 46L40 46L80 46M20)},
 % MRNUMBER = {996807 (90i:46104)},
%MRREVIEWER = {Masatoshi Enomoto},
       DOI = {\href{http://dx.doi.org/10.1090/memo/0424}{10.1090/memo/0424}},
}

\bib{Wil}{book}{%MR2288954,
    AUTHOR = {Williams, Dana P.},
     TITLE = {Crossed Products of C*-Algebras},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {134},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2007},
     PAGES = {xvi+528},
      ISBN = {978-0-8218-4242-3; 0-8218-4242-0},
  % MRCLASS = {46-02 (22D25 46L05 46L35 46L55 46L85)},
 % MRNUMBER = {2288954 (2007m:46003)},
%MRREVIEWER = {Jonathan M. Rosenberg},
}

\bib{Wil2}{thesis} {%MR2941447,
    AUTHOR = {Willis, Paulette Nicole},
     TITLE = {C*-Algebras of labeled graphs and $*$-commuting endomorphisms},
      NOTE = {Thesis (Ph.D.)--The University of Iowa},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2010},
     PAGES = {113},
      ISBN = {978-1124-07016-2},
  % MRCLASS = {Thesis},
 % MRNUMBER = {2941447},
}

\bib{Win}{article}{%MR2179780,
    AUTHOR = {Winter, Wilhelm},
     TITLE = {On topologically finite-dimensional simple C*-algebras},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {332},
      YEAR = {2005},
    NUMBER = {4},
     PAGES = {843--878},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L85 (19K14 46L05 46L35)},
 % MRNUMBER = {2179780 (2006i:46102)},
%MRREVIEWER = {Huaxin Lin},
       DOI = {\href{http://dx.doi.org/10.1007/s00208-005-0657-z}{10.1007/s00208-005-0657-z}},
}

\bib{Yee}{article} {%MR2301938,
    AUTHOR = {Yeend, Trent},
     TITLE = {Groupoid models for the C*-algebras of topological higher-rank graphs},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {57},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {95--120},
      ISSN = {0379-4024},
  % MRCLASS = {46L05 (22D25 46L55)},
 % MRNUMBER = {2301938 (2008f:46074)},
}

\bib{Zel}{article} {%MR0241994,
    AUTHOR = {Zeller-Meier, Georges},
     TITLE = {Produits crois\'{e}s d'une C*-alg\`{e}bre par un groupe d'automorphismes},
   JOURNAL = {J. Math. Pures Appl. (9)},
%  FJOURNAL = {Journal de Math\'ematiques Pures et Appliqu\'ees. Neuvi\`eme
 %             S\'erie},
    VOLUME = {47},
      YEAR = {1968},
     PAGES = {101--239},
      ISSN = {0021-7824},
%   MRCLASS = {46.65},
%  MRNUMBER = {0241994 (39 \#3329)},
%MRREVIEWER = {B. Russo},
}

\end{biblist}
%\end{bibdiv}
